$^{13}$C Hyperpolarization with Nitrogen-Vacancy Centers in Micro- and Nanodiamonds for Sensitive Magnetic Resonance Applications

Nuclear hyperpolarization is a known method to enhance the signal in nuclear magnetic resonance (NMR) by orders of magnitude. The present work addresses the $^{13}$C hyperpolarization in diamond micro- and nanoparticles, using the optically-pumped nitrogen-vacancy center (NV) to polarize $^{13}$C spins at room temperature. Consequences of the small particle size are mitigated by using a combination of surface treatment improving the $^{13}$C relaxation ($T_1$) time, as well as that of NV, and applying a technique for NV illumination based on a microphotonic structure. Monitoring the light-induced redistribution of the NV spin state populations with electron paramagnetic resonance, a strong polarization enhancement for the NV spin state is observed in a narrow spectral region corresponding to about 4\% of these defect centers. By combining adjustments to the `PulsePol' sequence and slow sample rotation, the NV-$^{13}$C polarization transfer rate is improved further. The hyperpolarized $^{13}$C NMR signal is observed in particles of 2 $\mu$m and 100 nm median sizes, with enhancements over the thermal signal (at 0.29 T magnetic field), of 1500 and 940, respectively. The present demonstration of room-temperature hyperpolarization anticipates the development of agents based on nanoparticles for sensitive magnetic resonance applications.

==> latexmkrc <==
$sub_doc_output = 'output-subdoc';

@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne ' ') && ($sub_doc_output ne '.') ) {

             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}
